A Bayesian Framework for Power System Components Identification

Having actual models for power system components (such as generators and loads or auxiliary equipment) is vital to correctly assess the power system operating state and to establish stability margins. However, power system operators often have limited information about the actual values for power system component parameters. Even when a model is available, its operating parameters and control settings are time-dependent and subject to real-time identification. Ideally, these parameters should be identified from measurement data, such as phasor measurement unit (PMU) signals. However, it is challenging to do this from the ambient measurements in the absence of transient dynamics since the signal-to-noise ratio (SNR) for such signals is not necessarily large. In this paper, we design a Bayesian framework for on-line identification of power system component parameters based on ambient PMU data, which has reliable performance for SNR as low as five and for certain parameters can give good estimations even for unit SNR. We support the framework with a robust and time-efficient numerical method. We illustrate the approach efficiency on a synchronous generator example.

==> ind_backup.tex <==
\newpage
\section{Induction motor model}

We start from a basic electromechanical model for induction machine. The equivalent resistance and reactance are is $R/\sigma$ and $X$, where $\sigma = 1- \omega_m/\omega_e$ is the motor slip. First, we write the voltage current relation:

\begin{equation}
    I=\frac{V}{(R/\sigma + j X)}
\end{equation}




The following small-signal model can be derived:
\begin{equation}\label{Yinduct}
i_d + j i_q = \frac{v_d + j v_q}{(R/\sigma_0 + j X)} + \frac{RV_0}{(R + j \sigma_0 X)^2} \delta \sigma 
\end{equation}


In order to express $\delta \sigma$ we turn to the mechanical equation for the rotor angular velocity $\omega_m$. It can be written as:
\begin{equation}\label{inddynmain}
J \dot{\omega}_m = \frac{P_e}{\omega_e} - T_m
\end{equation}
Here the electric power $P_e$ is given by the following expression:
\begin{equation}\label{indpe}
P_e = \frac{\sigma R V^2}{R^2 + \sigma^2 X^2}
\end{equation}
The motor steady-state power $P_{e0}$ is:
\begin{equation}\label{Pe0}
P_{e0} = \frac{\sigma_0 R V_0^2}{R^2 + \sigma_0^2 X^2}
\end{equation}
here the subscript $0$ indicates, as usually, the steady-state values of corresponding variables.



Multiplication of equation \eqref{inddynmain} by $\omega_{e0}$ and dividing it by $P_n$ gives: 
\begin{equation}\label{inddynpu}
    \frac{2 H}{\omega_{e0}}\dot{\omega}_m = \frac{\omega_{e0}}{\omega_e}p_e - p_m
\end{equation}
The numerical values for motor parameters are the following: $H=0.5$ s, $p_m=0.5$ p.u., $R=0.08$ p.u, $X=0.2$ p.u., $V_0=1$ p.u. With this parameters the steady-state value of motor slip is approximately $\sigma_0 \approx 0.04$. We remind, that $\omega_{e0}=2\pi 50$ rads/s. 





Assuming mechanical torque $T_m$ to be constant, we can write the following small-signal approximation:
\begin{equation}
J \dot{\delta \omega_m} = \frac{1}{\omega_{e0}}\delta P_e - \frac{P_{e0}}{\omega_{e0}^2}\delta \omega_e
\end{equation}
Or in the per unit form:
\begin{equation}
\dot{\delta \omega_m} = \frac{\omega_{e0}}{2H}\delta p_e - \frac{p_{e0}}{2H}\delta \omega_e
\end{equation}





Using \eqref{indpe} we can write $\delta P_e$ as:
\begin{equation}
\delta P_e = \frac{R(R^2-\sigma_0^2 X^2) V_0^2}{(R^2 + \sigma_0^2 X^2)^2}\delta \sigma + \frac{2\sigma_0 R V_0^2}{R^2 + \sigma_0^2 X^2}\frac{v_d}{V_0}
\end{equation}
This equation can be conveniently rewritten in terms of per unit electric power $p_{e0}=P_{e0}/P_n$ and equation \eqref{Pe0} for $P_{e0}$:
\begin{equation}
\delta p_e = p_{e0}\frac{(R^2-\sigma_0^2 X^2)}{R^2 + \sigma_0^2 X^2}\frac{\delta \sigma}{\sigma_0} + 2p_{e0}\frac{v_d}{V_0}
\end{equation}





Next, we have for mechanical frequency:

\begin{equation}
\delta \omega_m =(1-\sigma_0) \delta \omega_e - \omega_{e0}\delta \sigma 
\end{equation}
from which we can express the variation of the motor slip $\delta \sigma$:
\begin{equation}
\delta \sigma =(1-\sigma_0) \frac{\delta \omega_e}{\omega_{e0}} - \frac{\delta \omega_m}{\omega_{e0}} 
\end{equation}
Using expression for $\delta p_e$ we can write:
\begin{equation}\label{deltasigma}
\delta \sigma =-\frac{2\omega_{e0}p_{e0}}{\beta(s)}\frac{v_d}{V_0} + \frac{2H (1-\sigma_0) s^2 + p_{e0}s}{\beta(s)}\frac{v_q}{V_0}
\end{equation}
where we have made the following denotations:
\begin{equation}
\beta = 2H\omega_{e0} s + \frac{\omega_{e0}(R^2-\sigma_0^2 X^2)p_{e0}}{\sigma_0(R^2 + \sigma_0^2 X^2)}
\end{equation}
and also used the per unit power $p_{e0}=P_{e0}/P_n$ where $P_n$ is the nominal power for the system. The inertia time constant $H$ is given by the standard relation:
\begin{equation}
H = \frac{J \omega_{e0}^2}{2 P_n} 
\end{equation}
We also used the following relation:
\begin{equation}
V_0 \delta \omega_e = \dot{v}_q \equiv sv_q 
\end{equation}

Separating the real and imaginary parts in \eqref{Yinduct}, we have:
\begin{equation}
i_d = \frac{P_{e0}}{V_0^2}v_d + \frac{Q_{e0}}{V_0^2}v_q + \frac{R(R^2-\sigma_0^2 X^2) V_0}{(R^2 + \sigma_0^2 X^2)^2}\delta \sigma
\end{equation}
\begin{equation}
i_q = \frac{P_{e0}}{V_0^2}v_q - \frac{Q_{e0}}{V_0^2}v_d - \frac{2\sigma_0 R^2 X V_0}{(R^2 + \sigma_0^2 X^2)^2} \delta \sigma
\end{equation}

Let us now choose the per-unit system where $V_0=1$ and $P_{e0}=1$. Then, combining these equations with \eqref{deltasigma} we get the following expressions for admittance matrix:
\begin{equation}
Y_{dd} = 1 - \frac{2\omega_{e0}(R^2 - \sigma_0^2 X^2)}{\sigma_0^2 R \beta}
\end{equation}
\begin{equation}
Y_{dq} = q_{e0}+ \frac{[2H (\sigma_0-1) s^2 + s][R^2 - \sigma_0^2 X^2]}{\sigma_0^2 R \beta}
\end{equation}
\begin{equation}
Y_{qd} = -q_{e0}+ \frac{4 \omega_{e0} X}{\sigma_0 \beta}
\end{equation}
\begin{equation}
Y_{qq} = 1- \frac{2X[2H (\sigma_0-1) s^2 + s] }{\sigma_0 \beta}
\end{equation}


Suppose we have a system:
\begin{equation}
\dot{x} = A x + B u + \Gamma \dot{u}
\end{equation}
In Laplace space the derivative term $\dot{u}$ has the form $su(s)$. Let us now substitute it by the following term, that is called filtered derivative:
\begin{equation}
\frac{s}{\tau s+1}u
\end{equation}
where $\tau$ is some regularization time constant. Let us introduce the following additional variable $z$:
\begin{equation}
z=-\frac{1}{\tau s+1}u
\end{equation}
Then the following is true:
\begin{equation}
\frac{\tau s}{\tau s+1}u=z+u
\end{equation}
And we also have equation for $z$:
\begin{equation}
\dot{z}=-\frac{1}{\tau} z - \frac{1}{\tau} u 
\end{equation}



Steps for simulating dynamics of induction machine:

\begin{enumerate}
    \item Use \eqref{inddynpu} with electric power \eqref{indpe} and constant $p_m=0.5$ as dynamic equation.
    \item For $\sigma$ us the following formula: $\sigma = 1- \omega_m/\omega_e$
    
    \item Use the following representation for $V(t)= U(t) e^{j\theta(t)}$.
    
    \item The electric frequency $\omega_e$ is also a dynamic variable: $\omega_e - \omega_{e0} = \dot{\theta}$
    
    \item Instead of $\omega_e - \omega_{e0} = \dot{\theta}$ use the following representation:

\begin{equation}
\omega_e = \omega_{e0} + \frac{1}{\tau}z +  \frac{1}{\tau} \theta
\end{equation}
where variable $z$ satisfies the following equation:
\begin{equation}
\dot{z}=-\frac{1}{\tau} z - \frac{1}{\tau} \theta 
\end{equation}
    
    
Formulas for calculating steady-state real and reactie power:

\begin{equation}
    P + j Q = V_0 I_0^*
\end{equation}
    
    
\end{enumerate}




==> induction_motor_model.tex <==
\newpage
\section{Induction motor model}

We start from a basic electromechanical model for induction machine. The equivalent resistance and reactance are is $R/\sigma$ and $X$, where $\sigma = 1- \omega_m/\omega_e$ is the motor slip. First, we write the voltage current relation:

\begin{equation}
    I=\frac{V}{(R/\sigma + j X)}
\end{equation}




The following small-signal model can be derived:
\begin{equation}\label{Yinduct}
i_d + j i_q = \frac{v_d + j v_q}{(R/\sigma_0 + j X)} + \frac{RV_0}{(R + j \sigma_0 X)^2} \delta \sigma 
\end{equation}


In order to express $\delta \sigma$ we turn to the mechanical equation for the rotor angular velocity $\omega_m$. It can be written as:
\begin{equation}\label{inddynmain}
J \dot{\omega}_m = \frac{P_e}{\omega_e} - T_m
\end{equation}
Here the electric power $P_e$ is given by the following expression:
\begin{equation}\label{indpe}
P_e = \frac{\sigma R V^2}{R^2 + \sigma^2 X^2}
\end{equation}
The motor steady-state power $P_{e0}$ is:
\begin{equation}\label{Pe0}
P_{e0} = \frac{\sigma_0 R V_0^2}{R^2 + \sigma_0^2 X^2}
\end{equation}
here the subscript $0$ indicates, as usually, the steady-state values of corresponding variables.



Multiplication of equation \eqref{inddynmain} by $\omega_{e0}$ and dividing it by $P_n$ gives: 
\begin{equation}\label{inddynpu}
    \frac{2 H}{\omega_{e0}}\dot{\omega}_m = \frac{\omega_{e0}}{\omega_e}p_e - p_m
\end{equation}
The numerical values for motor parameters are the following: $H=0.5$ s, $p_m=0.5$ p.u., $R=0.08$ p.u, $X=0.2$ p.u., $V_0=1$ p.u. With this parameters the steady-state value of motor slip is approximately $\sigma_0 \approx 0.04$. We remind, that $\omega_{e0}=2\pi 50$ rads/s. 





Assuming mechanical torque $T_m$ to be constant, we can write the following small-signal approximation:
\begin{equation}
J \dot{\delta \omega_m} = \frac{1}{\omega_{e0}}\delta P_e - \frac{P_{e0}}{\omega_{e0}^2}\delta \omega_e
\end{equation}
Or in the per unit form:
\begin{equation}
\dot{\delta \omega_m} = \frac{\omega_{e0}}{2H}\delta p_e - \frac{p_{e0}}{2H}\delta \omega_e
\end{equation}





Using \eqref{indpe} we can write $\delta P_e$ as:
\begin{equation}
\delta P_e = \frac{R(R^2-\sigma_0^2 X^2) V_0^2}{(R^2 + \sigma_0^2 X^2)^2}\delta \sigma + \frac{2\sigma_0 R V_0^2}{R^2 + \sigma_0^2 X^2}\frac{v_d}{V_0}
\end{equation}
This equation can be conveniently rewritten in terms of per unit electric power $p_{e0}=P_{e0}/P_n$ and equation \eqref{Pe0} for $P_{e0}$:
\begin{equation}
\delta p_e = p_{e0}\frac{(R^2-\sigma_0^2 X^2)}{R^2 + \sigma_0^2 X^2}\frac{\delta \sigma}{\sigma_0} + 2p_{e0}\frac{v_d}{V_0}
\end{equation}





Next, we have for mechanical frequency:

\begin{equation}
\delta \omega_m =(1-\sigma_0) \delta \omega_e - \omega_{e0}\delta \sigma 
\end{equation}
from which we can express the variation of the motor slip $\delta \sigma$:
\begin{equation}
\delta \sigma =(1-\sigma_0) \frac{\delta \omega_e}{\omega_{e0}} - \frac{\delta \omega_m}{\omega_{e0}} 
\end{equation}
Using expression for $\delta p_e$ we can write:
\begin{equation}\label{deltasigma}
\delta \sigma =-\frac{2\omega_{e0}p_{e0}}{\beta(s)}\frac{v_d}{V_0} + \frac{2H (1-\sigma_0) s^2 + p_{e0}s}{\beta(s)}\frac{v_q}{V_0}
\end{equation}
where we have made the following denotations:
\begin{equation}
\beta(s) = 2H\omega_{e0} s + \frac{\omega_{e0}(R^2-\sigma_0^2 X^2)p_{e0}}{\sigma_0(R^2 + \sigma_0^2 X^2)}
\end{equation}
and also used the per unit power $p_{e0}=P_{e0}/P_n$ where $P_n$ is the nominal power for the system. The inertia time constant $H$ is given by the standard relation:
\begin{equation}
H = \frac{J \omega_{e0}^2}{2 P_n} 
\end{equation}
We also used the following relation:
\begin{equation}
V_0 \delta \omega_e = \dot{v}_q \equiv sv_q 
\end{equation}

Separating the real and imaginary parts in \eqref{Yinduct}, and assuming all current and voltage components are in per unit and $V_0=1$, we have:
\begin{equation}
i_d = p_{e0}v_d + q_{e0}v_q + \frac{R(R^2-\sigma_0^2 X^2)}{(R^2 + \sigma_0^2 X^2)^2}\delta \sigma
\end{equation}
\begin{equation}
i_q = p_{e0}v_q - q_{e0}v_d - \frac{2\sigma_0 R^2 X }{(R^2 + \sigma_0^2 X^2)^2} \delta \sigma
\end{equation}

Then, combining these equations with \eqref{deltasigma} we get the following expressions for admittance matrix:
\begin{equation}
Y_{dd} = p_{e0}\left[1 - \frac{2\omega_{e0}R(R^2 - \sigma_0^2 X^2)}{\beta(s)(R^2 + \sigma_0^2 X^2)^2}\right]
\end{equation}
\begin{equation}
Y_{dq} = q_{e0}+ \frac{R(R^2 - \sigma_0^2 X^2)}{(R^2 + \sigma_0^2 X^2)^2}\frac{2H (1-\sigma_0) s^2 + p_{e0}s}{\beta(s)}
\end{equation}
\begin{equation}
Y_{qd} = -q_{e0}+ \frac{2\sigma_0 R^2 X}{(R^2 + \sigma_0^2 X^2)^2}\frac{2 \omega_{e0}p_{e0}}{\beta(s)}
\end{equation}
\begin{equation}
Y_{qq} = p_{e0}- \frac{2\sigma_0 R^2 X}{(R^2 + \sigma_0^2 X^2)^2}\frac{2H (1-\sigma_0) s^2 + p_{e0}s}{\beta(s)}
\end{equation}


Suppose we have a system:
\begin{equation}
\dot{x} = A x + B u + \Gamma \dot{u}
\end{equation}
In Laplace space the derivative term $\dot{u}$ has the form $su(s)$. Let us now substitute it by the following term, that is called filtered derivative:
\begin{equation}
\frac{s}{\tau s+1}u
\end{equation}
where $\tau$ is some regularization time constant. Let us introduce the following additional variable $z$:
\begin{equation}
z=-\frac{1}{\tau s+1}u
\end{equation}
Then the following is true:
\begin{equation}
\frac{\tau s}{\tau s+1}u=z+u
\end{equation}
And we also have equation for $z$:
\begin{equation}
\dot{z}=-\frac{1}{\tau} z - \frac{1}{\tau} u 
\end{equation}



Steps for simulating dynamics of induction machine:

\begin{enumerate}
    \item Use \eqref{inddynpu} with electric power \eqref{indpe} and constant $p_m=0.5$ as dynamic equation.
    \item For $\sigma$ us the following formula: $\sigma = 1- \omega_m/\omega_e$
    
    \item Use the following representation for $V(t)= U(t) e^{j\theta(t)}$.
    
    \item The electric frequency $\omega_e$ is also a dynamic variable: $\omega_e - \omega_{e0} = \dot{\theta}$
    
    \item Instead of $\omega_e - \omega_{e0} = \dot{\theta}$ use the following representation:

\begin{equation}
\omega_e = \omega_{e0} + \frac{1}{\tau}z +  \frac{1}{\tau} \theta
\end{equation}
where variable $z$ satisfies the following equation:
\begin{equation}
\dot{z}=-\frac{1}{\tau} z - \frac{1}{\tau} \theta 
\end{equation}
    
    
Formulas for calculating steady-state real and reactive power:

\begin{equation}
    P + j Q = V_0 I_0^*
\end{equation}

One can derive the following expressions for steady-state per unit values of $p_{e0}$ and $q_{e0}$: 
\begin{equation}\label{Pe0pu}
p_{e0} = \frac{\sigma_0 R}{R^2 + \sigma_0^2 X^2}
\end{equation}
\begin{equation}\label{qe0pu}
q_{e0} = \frac{\sigma_0^2 X}{R^2 + \sigma_0^2 X^2}
\end{equation}
    
    
    
    
\end{enumerate}



